Uncertainty-aware Parameter-Efficient Self-training for Semi-supervised Language Understanding

The recent success of large pre-trained language models (PLMs) heavily hinges on massive labeled data, which typically produces inferior performance in low-resource scenarios. To remedy this dilemma, we study self-training as one of the predominant semi-supervised learning (SSL) approaches, which utilizes large-scale unlabeled data to generate synthetic examples. However, too many noisy labels will hurt the model performance, and the self-training procedure requires multiple training iterations making it more expensive if all the model parameters of the PLM are updated. This paper presents UPET, a novel Uncertainty-aware Parameter-Efficient self-Training framework to effectively and efficiently address the labeled data scarcity issue. Specifically, we incorporate Monte Carlo (MC) dropout in Bayesian neural network (BNN) to perform uncertainty estimation for the teacher model and then judiciously select reliable pseudo-labeled examples based on confidence and certainty. During the student training, we introduce multiple parameter-efficient learning (PEL) paradigms that allow the optimization of only a small percentage of parameters. We also propose a novel Easy-Hard Contrastive Tuning to enhance the robustness and generalization. Extensive experiments over multiple downstream tasks demonstrate that UPET achieves a substantial improvement in terms of performance and efficiency. Our codes and data are released at https: //github.com/wjn1996/UPET.

==> sections/bg.tex <==

\section{Background Knowledge}
\subsection{Parameter-Efficient Learning Paradigms}
\label{appendix:pet}
PEL aims to update the partial parameters of the PLM to improve the training efficiency~\cite{Mao2022UniPELT}.
% and $|W^*|\ll|W|$, where $|\cdot|$ denotes the number of parameters.
We first introduce three classic parameter-efficient methods. 

\noindent\textbf{Ptuning.}
Ptuning~\cite{Liu2021GPT} adds a continuous prompt into the input and uses a prompt encoder to realize parameterization.
Specifically, for each input sequence $X$, we have a task-specific prompt template $\mathcal{T}$ as follows:
\begin{equation*}
P_1,\cdots,P_I,X, \texttt{It was MASK}.
\end{equation*}
where $P_i$ is a prompt pseudo token (as proposed in~\citet{Liu2021GPT}), $I$ is the total number of pseudo tokens, and \texttt{MASK} is a special token as the placeholder for model output.

\noindent\textbf{Prefix-tuning.}
Prefix-tuning~\cite{Li2021Prefix} (it can also be viewed as P-tuning V2~\cite{Liu2021Ptuningv2}) extends the key and value matrix with new continuous vectors in each transformer layer. 
We also denote the length of the prefix vectors as $I$.

\noindent\textbf{Adapter.}
Adapter-tuning~\cite{Houlsby2019Parameter} designs multiple adapter networks into the transformer bloc, which can be viewed as two feed-forward projections.
Specifically, the adapters first project the original $d$-dimensional features into a smaller dimension, $m$, apply a nonlinearity, and then project back to $d$ dimensions. 
The total number of parameters added per layer, including biases, is $2md+d+m$. By setting $m\ll d$, we limit the number of parameters added per task.


We extend these methods into two paradigms, i.e. Head-Tuning and Prompt-Tuning. Head-Tuning aims to stack the prediction layer based on the CLS head, while Prompt-Tuning aims to reuse the pre-training objective of Masked Language Modeling (MLM) and predict by the well-designed template and verbalizer.
As shown in Figure~\ref{fig:parameter-efficient-overview}, we can unify all parameter-efficient methods with both Head-Tuning and Prompt-Tuning.

\subsection{Bayesian neural network (BNN)}
\label{appendix:bnn}
We provide a brief introduction to BNN~\cite{Mukherjee2020Uncertainty}.
Given a neural model $f^{W}$ and a training set $\mathcal{D}_{l}$, the parameters $W$ can be optimized by the posterior distribution $p(W|\mathcal{D}_{l})$.
In the inference stage, suppose that we aim to generate the label for the unlabeled example $X_i\in\mathcal{D}_{u}$, we can calculate the probability distribution by:
\begin{equation}
\begin{aligned}
p(y=c|X_i)=\int_{W}p(y=c|f^{W}(X_i)p(W|D_{u})dW.
\label{eql:bnn-probability}
\end{aligned}
\end{equation}
In other words, BNN averages over all the possible weights instead of directly optimizing for the weights~\cite{Mukherjee2020Uncertainty}. 
% Given a labeled dataset $\mathcal{D}_{l}$, the parameter can be optimized by the posterior distribution $p(W|\mathcal{D}_{l})$. 
% During model inference, given one unlabeled example $X_i\in\mathcal{D}_{u}$, the probability distribution of each example $X_i$ for class $c\in\mathcal{Y}$ is $p(y=c|X_i)=\int_{W}p(y=c|f^{W}(X_i)p(W|D_{u})dW$. 
Yet, it is intractable in practice for Eq.~\ref{eql:bnn-probability}, so that we can find a surrogate distribution to make the calculation tractable. 
Specifically, we consider $q_{\theta}(W)$ to be the dropout distribution~\cite{Srivastava2014Dropout} which aims to sample $T$ masked model weights from the current model. 
Hence, the approximate posterior for each unlabeled example is:
\begin{equation}
\begin{aligned}
p(y=c|X_i)\approx\frac{1}{T}\sum_{t=1}^{T}p(y=c|f^{\widetilde{W}_t}(X_i)),
\label{eql:bnn-posterior}
\end{aligned}
\end{equation}
where $\{\widetilde{W}_t\}_{t=1}^{T}\sim q_{\theta}(W)$ are the masked model weights.
% This posterior probability can also be regarded as the teacher's confidence that the tag of the example $X_i$ is $c\in\mathcal{Y}$. Based on the confidence, thus, we can obtain a pseudo-labeled dataset $\mathcal{D}_{p}=\{X_i, \widetilde{Y}_i\}_{i=1}^{N_u}$ that pseudo annotated on the unlabeled dataset $\mathcal{D}_{u}$. 

\subsection{Partially Huberised Cross-Entropy}
\label{appendix:phce}

Partially huberised cross-entropy loss (PHCE loss) can be used to alleviate the noisy label problem via a simple variant of gradient clipping for the classification loss (e.g. cross-entropy). 
Given one example $(x, y)$, the PHCE loss $\phi(x, y)$ is denoted as:
\begin{equation}
\begin{aligned}
\left\{
        \begin{array}{rcl}
        -\tau p_{W}(x, y)  
        + \log\tau + 1  & p_{W}(x, y)\leq 1/\tau; \\
        -\log p_{W}(x, y)     & p_{W}(x, y)>1/\tau; \\
        \end{array} 
    \right.
\label{eql:loss-phce-2}
\end{aligned}
\end{equation}
where $\tau>1$ is the hyper-parameter. Thus, the model learned by Eq.~\ref{eql:loss-phce-2} can be more robust to the noisy labeled tokens than the common cross-entropy.

\section{Self-training Procedure}
\label{appendix:algorithm}
We show the whole training procedure in Algorithm~\ref{alg:train}.
Specifically, we first use the original PLM $f^{W_0}$ to initialize a teacher model $f_{tea}^{W}$ (Algorithm~\ref{alg:train}, Line 1), and then fine-tune the teacher model over few-shot labeled data $\mathcal{D}_l$ (Algorithm~\ref{alg:train}, Line 2).
During the iteration process, we sample a subset unlabeled set $\mathcal{D}_u'$ from $\mathcal{D}_u$, and obtain model confidence and certainty for each unlabeled example $\widetilde{X}$ (Algorithm~\ref{alg:train}, Line 4).
Based on these factors, we can calculate the sampling weight for each unlabeled example and sample some reliable examples to form an easy set $\mathcal{D}_r$, and the rest is formed as a hard set $\mathcal{D}_h$ (Algorithm~\ref{alg:train}, Line 7-9).
During the student learning, we use the original PLM $f^{W_0}$ to initialize a student model $f_{stu}^{w^*}$, and use PHCE loss and Easy-Hard Contrastive Tuning to train the parameter-efficient student model over the pseudo-labeled examples (Algorithm~\ref{alg:train}, Line 6, 10-12). At last, we can copy the parameter of the student model to the teacher and repeat until convergence.
